Transformers to Learn Hierarchical Contexts in Multiparty Dialogue for Span-based Question Answering

We introduce a novel approach to transformers that learns hierarchical representations in multiparty dialogue. First, three language modeling tasks are used to pre-train the transformers, token- and utterance-level language modeling and utterance order prediction, that learn both token and utterance embeddings for better understanding in dialogue contexts. Then, multi-task learning between the utterance prediction and the token span prediction is applied to fine-tune for span-based question answering (QA). Our approach is evaluated on the FriendsQA dataset and shows improvements of 3.8% and 1.4% over the two state-of-the-art transformer models, BERT and RoBERTa, respectively.

==> tex/related.tex <==
\section{Related Work}
\label{sec:reated-work}
\citet{devlin_2019} introduced BERT, which was pre-trained from English Wikipedia and BookCorpus~\cite{zhu_2015} and significantly increased the performance of many downstream tasks. Unlike the original BERT that has the next sentence prediction task, \citet{liu_2019} introduced RoBERTa which was optimized from BERT with only dynamic masked language modeling task and more pre-training corpus including CC-News~\cite{nagel_2016}, OpenWebText~\cite{gokaslan_2019}, and STORIES~\cite{trinh_2018} and even longer time for pre-training to increase the performance of many downstream tasks again.

